Combinatorial Blocking Bandits with Stochastic Delays

Recent work has considered natural variations of the multi-armed bandit problem, where the reward distribution of each arm is a special function of the time passed since its last pulling. In this direction, a simple (yet widely applicable) model is that of blocking bandits, where an arm becomes unavailable for a deterministic number of rounds after each play. In this work, we extend the above model in two directions: (i) We consider the general combinatorial setting where more than one arms can be played at each round, subject to feasibility constraints. (ii) We allow the blocking time of each arm to be stochastic. We first study the computational/unconditional hardness of the above setting and identify the necessary conditions for the problem to become tractable (even in an approximate sense). Based on these conditions, we provide a tight analysis of the approximation guarantee of a natural greedy heuristic that always plays the maximum expected reward feasible subset among the available (non-blocked) arms. When the arms' expected rewards are unknown, we adapt the above heuristic into a bandit algorithm, based on UCB, for which we provide sublinear (approximate) regret guarantees, matching the theoretical lower bounds in the limiting case of absence of delays.

==> conclusion.tex <==
\section*{Conclusion}
Our work is the first, to the best of our knowledge, that studies the effect of local temporal correlations between player's actions and reward distributions in the generic setting of combinatorial bandits. In terms of hardness, we show that this interplay can lead to very hard combinatorial problems, where one cannot hope for an approximation algorithm of ratio better than $\Omega(k^{-1/2 + \epsilon})$. Interestingly, the above holds even for ``easy'' feasible sets of arms, where linear optimization can be done in polynomial time (e.g., shortest paths). From the design part, and given an $(\alpha, \beta)$-oracle for the underlying feasible set of arms, we show that when this set satisfies the hereditary property, there exists an $\frac{\alpha\beta}{1 + \alpha\beta}$-approximation algorithm (asymptotically). In the bandit setting, we provide a UCB-based variant of our algorithm for which we prove optimal $\frac{\alpha\beta}{1 + \alpha\beta}$-regret guarantees.
